A new interpretable unsupervised anomaly detection method based on residual explanation

Despite the superior performance in modeling complex patterns to address challenging problems, the black-box nature of Deep Learning (DL) methods impose limitations to their application in real-world critical domains. The lack of a smooth manner for enabling human reasoning about the black-box decisions hinder any preventive action to unexpected events, in which may lead to catastrophic consequences. To tackle the unclearness from black-box models, interpretability became a fundamental requirement in DL-based systems, leveraging trust and knowledge by providing ways to understand the model's behavior. Although a current hot topic, further advances are still needed to overcome the existing limitations of the current interpretability methods in unsupervised DL-based models for Anomaly Detection (AD). Autoencoders (AE) are the core of unsupervised DL-based for AD applications, achieving best-in-class performance. However, due to their hybrid aspect to obtain the results (by requiring additional calculations out of network), only agnostic interpretable methods can be applied to AE-based AD. These agnostic methods are computationally expensive to process a large number of parameters. In this paper we present the RXP (Residual eXPlainer), a new interpretability method to deal with the limitations for AE-based AD in large-scale systems. It stands out for its implementation simplicity, low computational cost and deterministic behavior, in which explanations are obtained through the deviation analysis of reconstructed input features. In an experiment using data from a real heavy-haul railway line, the proposed method achieved superior performance compared to SHAP, demonstrating its potential to support decision making in large scale critical systems.

==> chapters/experiments/dataset_tep.tex <==
%\subsubsection{Tenessee Eastman Process}
Tennessee Eastman Process (TEP) ~\citep{downs1993plant} is a popular benchmark dataset for anomaly detection, fault diagnosis and plant-wide control. TEP describes an industrial chemical process comprising of the following units: reactor, condenser, vapor-liquid separator, recycle compressor and product stripper. It has standard training and test data sets about  non-linear and dynamic operating conditions involving two simultaneous chemical reactions. Further details about the process at all can be found on ~\citep{downs1993plant} and datasets are available for download on reference ~\citep{DVN/6C3JR1_2017}. 

TEP data are composed by 53 features, being 12 manipulated and 41 measured variables (22 continuous process measurements and 19 composition measurements). There 21 possible states in which "0" is normal and the other are different fault types. There are 500 simulation runs with different random seeds along 500 time series records for training and 960 for test (containing normal and faulty events). Since this papers has primary focus to evaluate interpretability capacities (instead of prediction performance) on autoencoders, a strict sampling inspired on ~\citep{fan2017autoencoder} was done in order to define a suitable scope for the main purpose. Therefore, only faults [5, 10, 11, 13, 16, 17, 18, 19, 20] were considered in the detection task. The autoencoder was trained using only normal records with using the 22 continuous measurements and 11 manipulated features from 500 training records. The model was tested with 9600 samples, in which 960 are normal samples and 960 for each fault type.
